Democracy and Growth in the 21st Century

We find that, in the 21st century, democracy has persistent negative impacts on growth in GDP and night-time light intensity. This finding emerges from five different instrumental variable strategies that account for potential invalidity in some of the instruments. Our analysis also suggests a key mechanism: In this century, many electoral democracies shift toward populism and protectionism. These political changes weaken trade and investment, collectively dampening economic growth. Democracies also experienced lower growth in subjective life satisfaction among citizens. However, democracy causes slower growth in CO2 emissions and energy use, suggesting a trade-off between economic growth and socio-environmental performance.

==> supporting_files/coefs/capital_growth_iv3_nocontrols_coef.tex <==
-3.4\unskip

==> supporting_files/coefs/capital_growth_iv3_nocontrols_se.tex <==
0.7\unskip

==> supporting_files/coefs/explanation_controls2.tex <==
Columns 1, 3, 5, 7, 9, and 11 have no controls, while columns 2, 4, 6, 8, 10, and 12 include the following baseline controls: absolute latitude, mean temperature, mean precipitation, population density, median age, and diabetes prevalence. \unskip

==> supporting_files/coefs/explanation_n_ols.tex <==
N refers to the number of countries for which IVs (Table \ref{tab:2sls_tab1} Panel A), controls, and outcomes are available. \unskip

==> supporting_files/coefs/export_value_iv2_nocontrols_coef.tex <==
-142.8\unskip

==> supporting_files/coefs/export_value_iv2_nocontrols_coef_abs.tex <==
142.8\unskip

==> supporting_files/coefs/export_value_iv2_nocontrols_se.tex <==
28.1\unskip

==> supporting_files/coefs/import_value_iv5_nocontrols_coef_abs.tex <==
145.5\unskip

==> supporting_files/coefs/import_value_iv5_nocontrols_se.tex <==
31.0\unskip

==> supporting_files/coefs/manu_va_growth_iv5_nocontrols_coef_abs.tex <==
2.4\unskip

==> supporting_files/coefs/manu_va_growth_iv5_nocontrols_se.tex <==
0.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_col9_ols_coef.tex <==
245.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_col9_ols_coef_abs.tex <==
245.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_col9_ols_se.tex <==
48.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv1_nocontrols_coef.tex <==
355.0\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv1_nocontrols_coef_abs.tex <==
355.0\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv1_nocontrols_se.tex <==
63.0\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv1_withcontrols_coef.tex <==
418.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv1_withcontrols_coef_abs.tex <==
418.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv1_withcontrols_se.tex <==
92.7\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv2_nocontrols_coef.tex <==
357.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv2_nocontrols_coef_abs.tex <==
357.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv2_nocontrols_se.tex <==
62.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv2_withcontrols_coef.tex <==
376.3\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv2_withcontrols_coef_abs.tex <==
376.3\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv2_withcontrols_se.tex <==
24.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv3_nocontrols_coef.tex <==
294.5\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv3_nocontrols_coef_abs.tex <==
294.5\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv3_nocontrols_se.tex <==
74.8\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv3_withcontrols_coef.tex <==
323.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv3_withcontrols_coef_abs.tex <==
323.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv3_withcontrols_se.tex <==
45.3\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv4_nocontrols_coef.tex <==
420.7\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv4_nocontrols_coef_abs.tex <==
420.7\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv4_nocontrols_se.tex <==
120.8\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv4_withcontrols_coef.tex <==
405.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv4_withcontrols_coef_abs.tex <==
405.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv4_withcontrols_se.tex <==
65.8\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv5_nocontrols_coef.tex <==
277.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv5_nocontrols_coef_abs.tex <==
277.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv5_nocontrols_se.tex <==
60.4\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv5_withcontrols_coef.tex <==
340.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv5_withcontrols_coef_abs.tex <==
340.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv5_withcontrols_se.tex <==
38.2\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv6_nocontrols_coef.tex <==
341.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv6_nocontrols_coef_abs.tex <==
341.6\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv6_nocontrols_se.tex <==
48.8\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv6_withcontrols_coef.tex <==
379.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv6_withcontrols_coef_abs.tex <==
379.9\unskip

==> supporting_files/coefs/mean_death_per_million_20_22_iv6_withcontrols_se.tex <==
25.7\unskip

==> supporting_files/coefs/mean_deaths_per_million_20_22_iv2_nocontrols_coef.tex <==
745.7\unskip

==> supporting_files/coefs/mean_deaths_per_million_20_22_iv2_nocontrols_coef_abs.tex <==
745.7\unskip

==> supporting_files/coefs/mean_deaths_per_million_20_22_iv2_nocontrols_se.tex <==
134.1\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_col10_ols_coef.tex <==
-1.5\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_col10_ols_coef_abs.tex <==
1.6\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_col10_ols_se.tex <==
0.4\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_col9_ols_coef.tex <==
-1.6\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_col9_ols_coef_abs.tex <==
1.6\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_col9_ols_se.tex <==
0.3\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv1_nocontrols_coef.tex <==
-2.8\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv1_withcontrols_coef.tex <==
-5.1\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv1_withcontrols_coef_abs.tex <==
5.1\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv1_withcontrols_se.tex <==
3.6\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv2_nocontrols_coef.tex <==
-1.8\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv2_withcontrols_coef.tex <==
-1.3\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv2_withcontrols_coef_abs.tex <==
1.3\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv2_withcontrols_se.tex <==
0.6\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv3_nocontrols_coef.tex <==
-2.5\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv3_withcontrols_coef.tex <==
-3.2\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv3_withcontrols_coef_abs.tex <==
3.2\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv3_withcontrols_se.tex <==
1.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv4_nocontrols_coef.tex <==
-1.6\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv4_withcontrols_coef.tex <==
-3.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv4_withcontrols_coef_abs.tex <==
3.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv4_withcontrols_se.tex <==
1.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv5_nocontrols_coef.tex <==
-2.3\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv5_withcontrols_coef.tex <==
-2.7\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv5_withcontrols_coef_abs.tex <==
2.7\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv5_withcontrols_se.tex <==
0.5\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv6_nocontrols_coef.tex <==
-2.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv6_nocontrols_coef_abs.tex <==
2.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv6_nocontrols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv6_withcontrols_coef.tex <==
-2.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv6_withcontrols_coef_abs.tex <==
2.0\unskip

==> supporting_files/coefs/mean_g_night_light_2001_2013_iv6_withcontrols_se.tex <==
0.4\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_col10_ols_coef.tex <==
-1.2\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_col10_ols_se.tex <==
0.6\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_col9_ols_coef_abs.tex <==
1.6\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_col9_ols_se.tex <==
0.4\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_iv3_nocontrols_coef_abs.tex <==
1.8\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_iv4_nocontrols_coef_abs.tex <==
1.0\unskip

==> supporting_files/coefs/mean_growth_rate_2001_2019_iv5_nocontrols_coef_abs.tex <==
2.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_col10_ols_coef.tex <==
-0.7\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_col10_ols_coef_abs.tex <==
0.8\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_col10_ols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_col9_ols_coef_abs.tex <==
0.8\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_col9_ols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv1_nocontrols_coef.tex <==
-0.9\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv1_withcontrols_coef.tex <==
-0.9\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv1_withcontrols_coef_abs.tex <==
0.9\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv1_withcontrols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv2_nocontrols_coef_abs.tex <==
0.9\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv2_withcontrols_coef.tex <==
-1.0\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv2_withcontrols_coef_abs.tex <==
1.0\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv2_withcontrols_se.tex <==
0.1\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv3_nocontrols_coef_abs.tex <==
0.8\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv3_withcontrols_coef.tex <==
-0.7\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv3_withcontrols_coef_abs.tex <==
0.7\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv3_withcontrols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv4_nocontrols_coef_abs.tex <==
0.7\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv4_withcontrols_coef.tex <==
-0.6\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv4_withcontrols_coef_abs.tex <==
0.6\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv4_withcontrols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv5_nocontrols_coef_abs.tex <==
1.0\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv5_withcontrols_coef.tex <==
-0.8\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv5_withcontrols_coef_abs.tex <==
0.8\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv5_withcontrols_se.tex <==
0.2\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv6_nocontrols_coef.tex <==
-0.9\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv6_nocontrols_coef_abs.tex <==
0.9\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv6_nocontrols_se.tex <==
0.1\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv6_withcontrols_coef.tex <==
-1.0\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv6_withcontrols_coef_abs.tex <==
1.0\unskip

==> supporting_files/coefs/mean_growth_rate_2020_2022_iv6_withcontrols_se.tex <==
0.1\unskip

==> tables/new_files/table2.tex <==
\begin{center}
\begin{table}  \centering
  %\caption{2SLS Regression Estimates of Democracy's Effects}\label{tab:2sls} 
  \caption{2SLS and GMM Estimates of Democracy's Effects}\label{tab:2sls_tab1} 
  \footnotesize
  \begin{threeparttable}
  
  \begin{tabular}{@{\extracolsep{0pt}}lcccccccccccc} 
\hline 
\hline 
 & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline 
\multicolumn{13}{l}{\textbf{Panel A: Two-Stage Least Squares}} \\ 
\input{tables/new_files/table2_panelA}
\hline 
\multicolumn{13}{l}{\textbf{Panel B: Two-Step Efficient GMM}} \\ 
\input{tables/new_files/table2_panelB}
\hline 
% Panel titles
\multicolumn{13}{l}{\textbf{Panel C: IV Estimation with Potentially Invalid IVs}} \\ 
& \multicolumn{6}{c}{\textbf{I) Two-Stage Hard Thresholding}} & \multicolumn{6}{c}{\textbf{II) Searching-Sampling}}\\
% Separators for channel categories
\cmidrule(lr){2-7} \cmidrule(lr){8-13}
\input{extensions/tables/table2_invalid_iv_panelC}
\hline 
\hline 
\end{tabular} 
\begin{tablenotes} 
\item {\footnotesize {\textit{Notes:} Panel A reports the 2SLS estimates of democracy's effect on the mean GDP growth rate in 2001-2019, the mean nighttime light intensity growth rate in 2001-2013, and the mean GDP growth rate in 2020-2022, using five different IV strategies.  
\input{supporting_files/coefs/explanation_dem} 
\input{supporting_files/coefs/explanation_ivs} 
\input{supporting_files/coefs/explanation_se} 
The p-values, presented under the standard errors, are displayed as 0.00 if they are strictly smaller than the 0.005 threshold. The F-statistics are from the first-stage regressions of the IVs against the democracy index in 2019. The corresponding first-stage coefficients are in Appendix Table \ref{tab:first-stage}. 
The J-statistic (p-value) shows the p-value from the overidentification J test of the null hypothesis that the instruments are valid. A low p-value suggests that some of the instruments may be invalid. %A high p-value suggests that the instruments are likely valid.
\input{supporting_files/coefs/explanation_controls_all} 
\input{supporting_files/coefs/explanation_n}
Panel B reports the two-step efficient GMM estimates. Panel C reports the estimates of democracy's effect using two methods to allow for potentially invalid IVs. Columns 1–6 use two-stage hard thresholding to select valid IVs, and columns 7-12 use searching-sampling to select valid IVs. For potential IVs, columns 1–2 and 7–8 use the fraction speaking English and the fraction speaking European, columns 3–4 and 9–10 use the ability to grow crops and mine minerals, and columns 5–6 and 11–12 use all the IVs together.
\input{supporting_files/coefs/explanation_vars}}}
\end{tablenotes}
\end{threeparttable}
\end{table} 
\end{center}

==> tables/new_files/table_invalid_iv.tex <==
\begin{center}
\begin{table}  \centering
  \caption{2SLS Regression with Potentially Invalid Instruments}
  \label{tab:2sls_inv_iv} 
  \footnotesize
  \begin{threeparttable}
  
  \begin{tabular}{@{\extracolsep{0pt}}lcccccccccccc} 
\\[-1.8ex]\hline 
\hline
\\[-1.8ex]

% Panel titles
& \multicolumn{6}{c}{\textbf{I) Two-Stage Hard Thresholding}} & \multicolumn{6}{c}{\textbf{II) Searching-Sampling}}\\

% Separators for channel categories
\cmidrule(lr){2-7} \cmidrule(lr){8-13}

\\[-1.8ex] & (1) & (2) & (3) & (4) & (5) & (6) & (7) & (8) & (9) & (10) & (11) & (12)\\ 
\hline \\[-1.8ex] 

\input{extensions/tables/table2_invalid_iv_panelA}
\hline
\hline \\[-1.8ex] 
\end{tabular}

\begin{tablenotes} 
\item {\footnotesize {\textit{Notes:} Panel A reports the 2SLS estimates of democracy's effect on the mean GDP growth rate in 2001-2019, that in 2020-2022, and the mean
nighttime light intensity growth rate in 2001-2013 using five different IV strategies. Columns 1–6 use two-stage hard thresholding to select valid IVs, and columns 7-12 use searching-sampling to select valid IVs. \input{supporting_files/coefs/explanation_dem} For potential IVs, columns 1–2 and 7–8 use the fraction speaking English and the fraction speaking European, columns 3–4 and 9–10 use the ability to grow crops and mine minerals, and columns 5–6 and 11–12 use all the IVs together. The p-values are displayed as 0.00 if they are strictly smaller than the 0.005 threshold.  \input{supporting_files/coefs/explanation_controls}
\input{supporting_files/coefs/explanation_se} \input{supporting_files/coefs/explanation_vars}}}
\end{tablenotes}
\end{threeparttable}
\end{table} 
\end{center}
